Effects of Frustrated Surface in Heisenberg Thin Films

We study by extensive Monte Carlo (MC) simulations and analytical Green function (GF) method effects of frustrated surfaces on the properties of thin films made of stacked triangular layers of atoms bearing Heisenberg spins with an Ising-like interaction anisotropy. We suppose that the in-plane surface interaction $J_s$ can be antiferromagnetic or ferromagnetic while all other interactions are ferromagnetic. We show that the ground-state spin configuration is non linear when $J_s$ is lower than a critical value $J_s^c$. The film surfaces are then frustrated. In the frustrated case, there are two phase transitions related to disorderings of surface and interior layers. There is a good agreement between MC and GF results. In addition, we show from MC histogram calculation that the value of the ratio of critical exponents $\gamma/\nu$ of the observed transitions is deviated from the values of two and three Ising universality classes. The origin of this deviation is discussed with general physical arguments.

==> cover_letter.tex <==
October 17, 2006.

MS BU 10092  Ngo

Dear Editor,

 Please find herewith the revised version of the manuscript
 entittled "Effect of frustrated surface in Heisenberg thin film"
 by V. T. Ngo and H. T. Diep, which we resubmit for publication in
 Phys. Review B.

 In this new version, we have taken into account all the remarks
 of the referee. Please see our reply to the referee and the list of detailed
 modifications given below.

 Yours sincerely,

 H. T Diep

 REPLY TO THE REFEREE:  List of modifications

 We thank the referee for his important remarks both on the
 presentation and the results of our paper. In this new version, we have modified the paper
 according to his remarks. Here are our answer and modifications (in the order of
 his remarks):

 1. The old section V has been removed following the suggestion of
 the referee. The organization of sections has been changed accordingly
 (see last paragraph of
 the Introduction).

 2.  The error below Eq. 25 has been corrected (it reads now 80^2)

 3.  The value of the spin is 1/2. This is now indicated below Eq. 25
and new equation (26) is added.

4.  To explain the non-zero value of surface magnetization, we
added a phrase: "Note that between $T_1$ and $T_2$, the ordering
of the second layer acts as an external field on the first layer,
inducing therefore a small value of its magnetization.  A further
evidence of the existence of the surface transition will be
provided with the surface susceptibility in the MC results shown
below" while showing Fig. 3.

5. We added the size used in the simulations in the figure
captions.

6. We are sorry for the error. We have corrected the notation for
the system size: we replace N by L everywhere. The system size is
now LxLxN_z.

 7. This is the most important question of the referee:
 We added several discussions at the beginning and at the end of the section
 IV to explain the origin of the deviation of the obtained value
 of $\gamma/\nu$.  We have added 6 new references (ref 27 to 32).
 We hope that the referee is now convinced by our explanation.

 8. The conclusion has been slightly modified.  In particular, we
 show the interest of the model considered here by adding
" Finally, we note that in surface magnetism the low surface
magnetization experimentally
observed\cite{zangwill,bland-heinrich} has been generally
attributed to the effects of the reduction  of magnetic moments of
surface atoms and/or the surface-localized low-lying magnon modes.
The model considered in this paper adds another origin for the low
surface magnetization: surface frustration.  It completes the list
of possible explanations for experimental observations in thin
films."

 9. The abstract has been modified to take into account the new
 modifications of the revised version.

 We believe that the revised version is now suitable for
 publication.

